From fractions to complete Segal spaces

We show that the Rezk classification diagram of a relative category admitting a homotopical version of the two-sided calculus of fractions is a Segal space up to Reedy-fibrant replacement. This generalizes the result of Rezk and Bergner on the classification diagram of a closed model category, as well as the result of Barwick and Kan on the classification diagram of a partial model category.

==> Prelude0.tex <==
\usepackage[T1]{fontenc} 
\usepackage[utf8]{inputenc}

\ifdefined\ifdraftdoc

\else
  \usepackage{ifdraft}
  \makeatletter
  \let\ifdraftdoc\if@draft
  \makeatother
\fi

\usepackage{needspace}

\usepackage{multirow}
\usepackage[leqno]{amsmath}
\allowdisplaybreaks[4]
\usepackage{amsthm}
\usepackage{amssymb}
\usepackage{amsfonts}

\renewcommand{\qedsymbol}{$\blacksquare$}
\newcommand{\openqedsymbol}{$\square$}
\newcommand{\exercisesymbol}{$\lozenge$}
\newcommand{\obvioussymbol}{$\blacklozenge$}
\newcommand{\openproof}{\renewcommand{\qedsymbol}{\openqedsymbol}}
\newcommand{\exerproof}{\renewcommand{\qedsymbol}{\exercisesymbol}}
\newcommand{\obviousproof}{\renewcommand{\qedsymbol}{\obvioussymbol}}

\usepackage{mathrsfs}
\DeclareMathAlphabet{\mathcal}{OMS}{cmsy}{m}{n}
\usepackage{stmaryrd}

\usepackage{mathtools}

\usepackage[english]{babel}

\usepackage[autostyle]{csquotes}
\usepackage{hyphenat}

\usepackage{etoolbox}
\usepackage{xstring}

\usepackage[shortlabels]{enumitem}

\usepackage[dvipsnames,hyperref]{xcolor}

\usepackage{tikz}
\usepackage{tikz-cd}

\usetikzlibrary{arrows, shapes.geometric}
\usetikzlibrary{decorations.pathmorphing}
\tikzset{baseline=(current bounding box.center)}

\let\LiningNumbers\relax

\linespread{1.1}

\DeclareTextFontCommand{\textrmup}{\rmfamily\mdseries\upshape}
\DeclareTextFontCommand{\textbfup}{\rmfamily\bfseries\upshape}
\DeclareTextFontCommand{\textttup}{\ttfamily\mdseries\upshape}
\DeclareTextFontCommand{\textsfup}{\sffamily\mdseries\upshape}

\setlist[enumerate]{font=\upshape}

\DeclareFontFamily{OT1}{pzc}{}
\DeclareFontShape{OT1}{pzc}{mb}{it}{
   <-> s * [1.150] pzcmi7t
}{}

\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{mb}{it}

\DeclareMathSymbol{\epsilon}{\mathord}{letters}{"22}
\DeclareMathSymbol{\phi}{\mathord}{letters}{"27}
\DeclareMathSymbol{\varepsilon}{\mathord}{letters}{"0F}
\DeclareMathSymbol{\varphi}{\mathord}{letters}{"1E}

\usepackage{microtype}

\makeatletter
\newcommand*{\noprelistbreak}{\@nobreaktrue\nopagebreak}
\makeatother

\usepackage{xspace}

\newcommand{\hairspace}{\ifmmode\mskip1mu\else\kern0.08em\fi}
\newcommand{\mmhfill}{\hskip \textwidth minus \textwidth}

\makeatletter
\def\abbrdot{\@ifnextchar.{}{.\@\xspace}}
\makeatother
\newcommand{\etc}{etc\abbrdot}
\newcommand{\eg}{e.g\abbrdot}
\newcommand{\ie}{i.e\abbrdot}
\newcommand{\resp}{resp\abbrdot}
\newcommand{\confer}{cf\abbrdot}
\newcommand{\loccit}{loc.\@ cit\abbrdot}
\newcommand{\opcit}{op.\@ cit\abbrdot}

\newcommand{\Chap}{Ch.\@~}
\newcommand{\Appx}{App.\@~}
\newcommand{\Sect}{\S\hairspace}
\newcommand{\Sects}{\S\S\hairspace}
%\newcommand{\textnumero}{N\textsuperscript{\underline{o}}\xspace}
\newcommand{\Numero}{N\textsuperscript{\underline{o}}~}

\newcommand{\strong}[1]{\textbfup{#1}}

\renewcommand{\implies}{\ifmmode\Longrightarrow\else$\Rightarrow$\expandafter\xspace\fi}
\renewcommand{\iff}{\ifmmode\Longleftrightarrow\else$\Leftrightarrow$\expandafter\xspace\fi}

\makeatletter
\let\internal@prime\prime
\renewcommand{\prime}{\ifmmode\internal@prime\else$\sp{\internal@prime}$\expandafter\xspace\fi}
\makeatother

\renewcommand{\lnot}{\mathord{\neg}}

\ifdefined\nequiv

\else
  \def\nequiv{\not\equiv}
\fi

\newcommand{\join}{\vee}
\newcommand{\meet}{\wedge}

\newcommand{\blank}{\mathord{-}}
\newcommand{\pblank}{\mathord{(-)}}

\newcommand{\bcirc}{\bullet}

\newcommand{\embedinto}{\hookrightarrow}
\newcommand{\hoto}{\Rightarrow}

\makeatletter
\newcommand{\profto}{\mathrel{\mathpalette\profto@int\relax}}
\newcommand{\profto@int}[2]{\ooalign{$#1\rightarrow$\cr\hfil$#1\mapsfromchar$\hfil\cr}}
\makeatother

\newcommand{\sharplylt}{\vartriangleleft}

\DeclareMathSymbol{.}{\mathpunct}{letters}{"3A}
\DeclareMathSymbol{:}{\mathrel}{operators}{"3A}

\DeclareMathOperator{\ob}{ob}
\DeclareMathOperator{\mor}{mor}
\DeclareMathOperator{\iso}{iso}

\DeclareMathOperator{\und}{und}
\DeclareMathOperator{\weq}{weq}

\newcommand{\cotens}{\mathbin{\pitchfork}}

\DeclareMathOperator{\discr}{disc}

\newcommand{\Ho}[1][]{\mathop{\mathrm{Ho}\ifstrempty{#1}{}{\sb{#1}}}}

\newcommand{\LH}{\mathbf{L}^\mathrm{H}}

\DeclareMathOperator{\dom}{dom}
\DeclareMathOperator{\codom}{codom}

\let\prolim\varprojlim
\let\indlim\varinjlim

\newcommand{\id}{\mathrm{id}}

\AtBeginDocument{\let\emptyset\varnothing}

\newcommand*{\lr}[3]{\mathopen{}\mathclose{\left#1{#2}\right#3}}
\newcommand*{\lmr}[5]{\mathopen{}\mathclose{\left#1{#2}\,\middle#3\,{#4}\right#5}}
\newcommand*{\lrsmash}[3]{\lr#1{\smash{#2}}#3}
\newcommand*{\smashlr}[3]{\mathopen{}\smash{\lr#1{#2}#3}\mathclose{}}
\newcommand*{\ordlr}[3]{\mathord{\left#1{#2}\right#3}}
\newcommand*{\argp}[1]{\ifstrempty{#1}{}{\lr({#1})}}
\newcommand*{\argptwo}[2]{\lr({#1, #2})}
\newcommand*{\argptwotwo}[4]{\lr({#1, #2; #3, #4})}
\newcommand*{\argb}[1]{\ifstrempty{#1}{}{\lr[{#1}]}}
\newcommand*{\parens}[1]{\lr({#1})}
\newcommand*{\ordparens}[1]{\ordlr({#1})}
\newcommand*{\bracket}[1]{\lr[{#1}]}
\newcommand*{\qquote}[1]{\lr\ulcorner{#1}\urcorner}
\newcommand*{\abs}[1]{\ordlr|{#1}|}
\newcommand*{\tuple}[1]{\ordlr({#1})}
\newcommand*{\tuplesmash}[1]{\mathord{\lrsmash({#1})}}
\newcommand*{\prodtuple}[1]{\lr<{#1}>}
\newcommand*{\coprodtuple}[1]{\lr({#1})}

\newcommand*{\setbuilder}[2]{\mathord{\lmr\{{#1}|{#2}\}}}
\newcommand*{\seqbuilder}[2]{\mathord{\lmr({#1}|{#2})}}

\ifdefined\fracslash

\else
  \def\fracslash{\mathbin{/}}
\fi
\ifdefined\divslash

\else
  \def\divslash{\mathbin{/}}
\fi

\newcommand*{\ul}[1]{\smash{\underline{#1}}\vphantom{#1}}

\renewcommand{\vec}[1]{\mathbf{#1}}
%\makeatletter
%\let\vec@int\vec
%\renewcommand*{\vec}[1]{\smash{\vec@int{#1}}\vphantom{#1}}
%\makeatother

\makeatletter
\newcommand*{\optargp}{\new@ifnextchar\bgroup{\argp}{}}
\newcommand*{\optargptwo}{\new@ifnextchar\bgroup{\expandafter\optargptwo@first}{}}
\newcommand*{\optargptwo@first}[1]{\new@ifnextchar\bgroup{\argptwo{#1}}{\argp{#1}}}
\newcommand*{\optargptwotwo}{\new@ifnextchar\bgroup{\expandafter\optargptwotwo@first}{}}
\newcommand*{\optargptwotwo@first}[2]{\new@ifnextchar\bgroup{\argptwotwo{#1}{#2}}{\argptwo{#1}{#2}}}

\newcommand*{\sbtwo}[2]{\sb{\lr({{#1}, {#2}})}}

\newcommand*{\optsb}{\new@ifnextchar\bgroup{\sb}{}}
\newcommand*{\optsp}{\new@ifnextchar\bgroup{\sp}{}}
\newcommand*{\optsbtwo}{\new@ifnextchar\bgroup{\expandafter\optsbtwo@first}{}}
\newcommand*{\optsbtwo@first}[1]{\new@ifnextchar\bgroup{\sbtwo{#1}}{\sb{#1}}}

\newcommand*{\bracketoptsb}[1][]{\sb{#1}}
\newcommand*{\bracketoptsp}[1][]{\sp{#1}}

\newcommand*{\optsbargp}[1][]{\sb{#1}\optargp}
\newcommand*{\optspargp}[1][]{\sp{#1}\optargp}
\newcommand*{\optsbspargp}[1][]{\sb{#1}\optspargp}
\newcommand*{\optspsbargp}[1][]{\sp{#1}\optsbargp}

\newcommand*{\optsbargptwo}[1][]{\sb{#1}\optargptwo}
\newcommand*{\optspargptwo}[1][]{\sp{#1}\optargptwo}
\newcommand*{\optsbspargptwo}[1][]{\sb{#1}\optspargptwo}
\newcommand*{\optspsbargptwo}[1][]{\sp{#1}\optsbargptwo}

\newcommand*{\set}[1]{\new@ifnextchar\bgroup{\setbuilder{#1}}{\ordlr\{{#1}\}}}
\newcommand*{\seq}[1]{\new@ifnextchar\bgroup{\seqbuilder{#1}}{\tuple{#1}}}
\makeatother

\ifdefined\hash

\else
  \def\hash{\#}
\fi
\newcommand*{\card}[1]{\lr|{#1}|}
\ifdefined\powerset
  \undef\powerset
\else

\fi
\newcommand*{\powerset}[1][]{\mathscr{P}\ifstrempty{#1}{\hairspace}{\sb{#1}} \optargp}

\newcommand{\mbfs}{\mathbf{s}}
\newcommand{\mbfc}{\mathbf{c}}

\newcommand*{\smashsp}[2]{{#1}\sp{\smash{#2}}}

\newcommand*{\subdiv}[1]{\smashsp{#1}{\textrmup{\S}}}

\newcommand*{\op}[1]{\smashsp{#1}{\mathrm{op}}}
\newcommand*{\co}[1]{\smashsp{#1}{\mathrm{co}}}
\newcommand*{\coop}[1]{\smashsp{#1}{\mathrm{co\hairspace op}}}

\newcommand*{\inv}[2][1]{{#2}^{-#1}}

\makeatletter
\newcommand*{\ctchoice}[2]{%
  \ifdef{\ct@homstyle}%
  {#2}%
  {#1}}
\newcommand*{\ctchoicetwo}[5]{%
  \ifdef{\ct@homcatstyle}%
  {#2}{%
  \ifdef{\ct@transfstyle}%
  {#3}{%
  \ifdef{\ct@catstyle}%
  {#4}{%
  \ifdef{\ct@homstyle}%
  {#5}{%
  {#1}}}}}}
  
\newcommand*{\DefineCategory}[2]{\DeclareRobustCommand{#1}{\ctchoice{\mathbf{#2}}{\mathbf{#2}}}}
\newcommand*{\DefineBicategory}[2]{\DeclareRobustCommand{#1}{\ctchoicetwo{\mathfrak{#2}}{\mathfrak{#2}}{\mathfrak{#2}}{\mathbf{#2}}{\mathbf{#2}}}}

\newcommand*{\cat}[1]{%
  \begingroup%
  \def\ct@catstyle{cat}%
  #1%
  \endgroup}
\newcommand*{\bicat}[1]{%
  \begingroup
  \def\ct@bicatstyle{bicat}%
  #1%
  \endgroup}
\newcommand*{\Hom}[1][]{%
  \begingroup%
  \def\ct@homstyle{hom}%
  \ifstrempty{#1}{\mathrm{Hom}}{#1}%
  \endgroup%
  \optargptwo}
\newcommand*{\HHom}[1][]{%
  \begingroup%
  \def\ct@homcatstyle{homcat}%
  \ifstrempty{#1}{\mathbf{Hom}}{#1}%
  \endgroup
  \optargptwo}
\newcommand*{\hpty}[1][]{%
  \begingroup%
  \def\ct@transfstyle{transf}%
  \ifstrempty{#1}{\mathrm{Nat}}{#1}%
  \endgroup
  \optargptwotwo}

\makeatother

\DefineCategory{\Set}{Set}
\newcommand{\FinSet}{\ctchoice{\mathbf{FinSet}}{\mathbf{Set}}}

\DefineCategory{\Simplex}{\Delta}
\DefineCategory{\SSet}{sSet}
\DefineCategory{\SSSet}{ssSet}

\newcommand{\Cat}{\ctchoicetwo{\mathfrak{Cat}}{\mathbf{Fun}}{\mathbf{Fun}}{\mathbf{Cat}}{\mathrm{Fun}}}

\newcommand*{\commacat}[2]{\ordlr({#1 \mathbin{\downarrow} #2})}
\newcommand*{\isocommacat}[2]{\ordlr({#1 \mathbin{\wr} #2})}

\newcommand*{\slicecat}[2]{\mathord{#1 \mathord{\divslash} #2}}
\newcommand*{\overcat}[2]{\mathord{#1 \sb{\mathord{\divslash} #2}}}
\newcommand*{\undercat}[2]{\mathord{\sp{#1 \mathord{\divslash}} #2}}

\newcommand*{\nv}[1][]{\mathrm{N}\sp{#1}\optargp}
\newcommand*{\Nv}[1][]{\mathbf{N}\sp{#1}\optargp}
\newcommand*{\rn}[2][]{\ordlr|{#2}|\ifstrempty{#1}{}{\sb{#1}}}
\DeclareMathOperator{\Tot}{Tot}
\newcommand*{\Groth}[3]{\mathbf{G}\argp{{#1}, {#2}, {#3}}}

\newcommand{\skel}[1][]{\mathrm{sk}\sb{#1}\optargp}
\newcommand{\coskel}[1][]{\mathrm{cosk}\sb{#1}\optargp}
\newcommand{\cskel}[1][]{\mathrm{sk}\sp{#1}\optargp}
\newcommand{\ccoskel}[1][]{\mathrm{cosk}\sp{#1}\optargp}

\newcommand{\totalL}{\mathbf{L}}
\newcommand{\totalR}{\mathbf{R}}
\newcommand{\pointL}{\mathbb{L}}
\newcommand{\pointR}{\mathbb{R}}

\newcommand*{\Cocyc}[1][]{\ifstrempty{#1}{{\mathbb{H}}^{{\sim}{\to}}}{{#1}^{\bracket{-1 ; 1}}}\optsbargptwo}

\newcommand*{\homs}{\mathpzc{h}\optsb}

\newcommand*{\sHom}[1][]{\ifstrempty{#1}{\smash{\mathpzc{Hom}}\vphantom{\mathrm{Hom}}}{\smash{\mathpzc{Hom}}\vphantom{\mathrm{Hom}}_{#1}}\optargptwo}
\newcommand*{\RHom}[1][]{\ifstrempty{#1}{\totalR \mathrm{Hom}}{\totalR \mathrm{Hom}_{#1}}\optargptwo}

\newcommand*{\xHom}[3][]{\ifstrempty{#1}{\ordlr[{{#2}, {#3}}]}{\ordlr[{{#2}, {#3}}]\sb{#1}}}
\newcommand*{\ulHom}[1][]{\ifstrempty{#1}{\ul{\Hom}}{\ul{\Hom[#1]}}\optargptwo}

\newcommand*{\Ext}{\mathrm{Ext}\optspsbargptwo}

\newcommand*{\eval}[1][]{\ifstrempty{#1}{\mathrm{ev}}{\mathrm{ev}_{#1}}\optargptwo}

\newcommand*{\Func}[2]{\xHom{#1}{#2}}
\let\RelFun\Func
%\newcommand*{\RelFun}[2]{\xHom[\mathrm{h}]{#1}{#2}}

\newcommand*{\kwlim}[3][]{\ordlr\lbrace{{#2}, {#3}}\rbrace\sp{#1}}
\newcommand*{\kwcolim}[3][]{{#2} \mathbin{\star\sb{#1}} {#3}}

\newcommand*{\wlim}[2][]{\mathchoice%
  {\mathop{{\varprojlim}^{#2}}_{{#1}\phantom{#2}}}%
  {\varprojlim_{#1}^{#2}}%
  {\varprojlim_{#1}^{#2}}%
  {\varprojlim_{#1}^{#2}}}
\newcommand*{\wcolim}[2][]{\mathchoice%
  {\mathop{{\varinjlim}^{#2}}_{{#1}\phantom{#2}}}%
  {\varinjlim_{#1}^{#2}}%
  {\varinjlim_{#1}^{#2}}%
  {\varinjlim_{#1}^{#2}}}

\newcommand{\hocolim}[1][]{\mathop{\mathrm{ho}{\varinjlim}}_{#1}}
\newcommand{\BKcolim}[1][]{\wcolim[#1]{\mathrm{BK}}}
\newcommand{\KBcolim}[1][]{\wcolim[#1]{\mathrm{KB}}}
\newcommand{\laxcolim}[1][]{\wcolim[#1]{\mathrm{Th}}}
\newcommand{\oplaxcolim}[1][]{\wcolim[#1]{\mathrm{Gr}}}

\newcommand{\Path}{\mathrm{Path} \optargp}

\usepackage[colorlinks,linkcolor=Blue,citecolor=Blue,urlcolor=blue,pdfpagelabels,pdffitwindow=false]{hyperref}

\usepackage{thmtools}

\declaretheorem[style=plain,parent=section,title=Theorem,refname=theorem,Refname=Theorem]{thm}
\declaretheorem[style=plain,sibling=thm,title=Proposition,refname=proposition,Refname=Proposition]{prop}
\declaretheorem[style=plain,sibling=thm,title=Lemma,refname=lemma,Refname=Lemma]{lem}
\declaretheorem[style=plain,sibling=thm,title=Corollary,refname=corollary,Refname=Corollary]{cor}

\declaretheorem[style=definition,sibling=thm,title=Definition,refname=definition,Refname=Definition]{dfn}

\declaretheorem[style=definition,sibling=thm,title=Example,refname=example,Refname=Example]{example}
\declaretheorem[style=definition,sibling=thm,title=Examples,refname=examples,Refname=Examples]{examples}
\declaretheorem[style=definition,qed=\exercisesymbol,sibling=thm,title=Exercise,refname=exercise,Refname=Exercise]{exercise}

\declaretheoremstyle[style=remark,headfont=\scshape]{remark}
\declaretheorem[style=remark,sibling=thm,title=Remark,refname=remark,Refname=Remark]{remark}

\declaretheorem[style=plain,numbered=no,title=Theorem]{thm*}
\declaretheorem[style=plain,numbered=no,title=Proposition]{prop*}
\declaretheorem[style=remark,numbered=no,title=Remark]{remark*}
\declaretheorem[style=definition,numbered=no,title=Example]{example*}

\def\chapterAutorefname{Chapter}

\makeatletter
\@counteralias{numpar}{thm}
\def\numparAutorefname{Paragraph}
\def\numparautorefname{paragraph}
\newcommand*{\makenumpar}[1][]{%
  \par%
  \refstepcounter{numpar}%
  {\normalfont{\bfseries\textparagraph}\hspace{0.5em}\thenumpar\ifstrempty{#1}{}{ ({\normalfont #1})}.} }
\makeatother

\AtBeginDocument{%
\hyphenation{pull-back pull-backs push-out push-outs co-pro-duct co-pro-ducts co-com-plete sub-ob-ject sub-ob-jects more-over quasi-com-pact de-gen-er-ate pro-vided Gro-then-dieck Law-vere mod-ule sub-al-ge-bra fi-brant co-fi-brant fi-brant-ly co-fi-brant-ly bi-cat-e-go-ry bi-cat-e-gor-ic-al bi-cat-e-gor-ic-al-ly qua-si-cat-e-go-ry qua-si-cat-e-go-ries qua-si-cat-e-go-ric-al}%
}

==> PreludeA.tex <==
\input{Prelude0}

\makeatletter
\renewcommand\footnoterule{%
  \vfill
  \kern-3\p@
  \hrule\@width.4\columnwidth
  \kern2.6\p@}

\renewcommand*{\@makefnmark}{\hbox{\textsuperscript{\normalfont [\LiningNumbers\@thefnmark]}}}
\renewcommand*{\@makefntext}[1]{\parindent 1.0em\noindent\ifdefempty{\@thefnmark}{}{\hb@xt@-1.0em{\hss \normalfont [\LiningNumbers \@thefnmark]}\hspace{1.0em}}#1}
\HyOrg@addtoreset{footnote}{chapter}
\newcommand{\footpar}[1]{\gdef\@thefnmark{}\@footnotetext{#1}}

\newcommand{\hangsecnum}{\def\@seccntformat##1{\llap{\csname the##1\endcsname\quad}}}
\makeatother

\usepackage[natbib,safeinputenc,backend=biber,style=authoryear-comp,bibstyle=authoryear]{biblatex}

\DeclareSortingScheme{mysort}{
  \sort{
    \field{presort}
  }
  \sort[final]{
    \field{sortkey}
  }
  \sort{
    \name{sortname}
    \name{author}
    \name{editor}
    \name{translator}
    \field{sorttitle}
    \field{title}
  }
  \sort{
    \field{sortyear}
    \field{year}
  }
  \sort{
    \field{month}
  }
  \sort{
    \field{day}
  }
  \sort{
    \field{journal}
  }
  \sort{
    \field[padside=left,padwidth=4,padchar=0]{volume}
    \literal{0000}
  }
  \sort{
    \field{series}
  }
  \sort{
    \field[padside=left,padwidth=4,padchar=0]{number}
    \literal{0000}
  }
  \sort{
    \field{sorttitle}
    \field{title}
  }
}

\ExecuteBibliographyOptions{sorting=mysort,block=space,useprefix=true,maxcitenames=3,maxbibnames=10,mergedate=false,pagetracker=false}

%%% BEGIN BibLaTeX style

\setlength{\bibnamesep}{\baselineskip}
\renewcommand*{\bibnamedash}{}
\newcommand*{\authoryearpunct}{\hspace*{-\bibhang}\bibsentence}
\renewcommand*{\labelnamepunct}{\addspace}

\makeatletter

\appto\citesetup{\LiningNumbers}

\renewbibmacro*{cite:label}{%
  \iffieldundef{label}
    {\printtext[bibhyperref]{\printfield[citetitle]{labeltitle}}}
    {\printtext[bibhyperref]{\printfield{label}}}}

\renewbibmacro*{date+extrayear}{%
  \iffieldundef{shorthand}
    {\iffieldundef{labelyear}
      {}
      {\printtext[brackets]{\printfield{labelyear}\printfield{extrayear}}}\addspace}
    {\printtext[brackets]{\printfield{shorthand}}}}

\renewbibmacro*{author}{%
  \ifboolexpr{
    test \ifuseauthor
    and
    not test {\ifnameundef{author}}
  }
    {\usebibmacro{bbx:dashcheck}
       {\bibnamedash}
       {\usebibmacro{bbx:savehash}%
        \printnames{author}%
    \newline\setunit{\authoryearpunct}}%
     \iffieldundef{authortype}
       {}
       {\usebibmacro{authorstrg}%
    \setunit{\addspace}}}%
    {\global\undef\bbx@lasthash
     \usebibmacro{labeltitle}%
     \setunit*{\addspace}}%
  \usebibmacro{date+extrayear}}

\renewbibmacro*{bbx:editor}[1]{%
  \ifboolexpr{
    test \ifuseeditor
    and
    not test {\ifnameundef{editor}}
  }
    {\usebibmacro{bbx:dashcheck}
       {\bibnamedash}
       {\printnames{editor}%
    \newline\setunit{\authoryearpunct}%
    \usebibmacro{bbx:savehash}}%
     \usebibmacro{#1}%
     \clearname{editor}%
     \setunit{\addspace}}%
    {\global\undef\bbx@lasthash
     \usebibmacro{labeltitle}%
     \setunit*{\addspace}}%
  \usebibmacro{date+extrayear}}

\renewbibmacro*{bbx:translator}[1]{%
  \ifboolexpr{
    test \ifusetranslator
    and
    not test {\ifnameundef{translator}}
  }
    {\usebibmacro{bbx:dashcheck}
       {\bibnamedash}
       {\printnames{translator}%
    \newline\setunit{\authoryearpunct}%
    \usebibmacro{bbx:savehash}}%
     \usebibmacro{translator+othersstrg}%
     \clearname{translator}%
     \setunit{\addspace}}%
    {\global\undef\bbx@lasthash
     \usebibmacro{labeltitle}%
     \setunit*{\addspace}}%
  \usebibmacro{date+extrayear}}

\makeatother

%%% END BibLaTeX style

\renewcommand*{\mkbibparens}[1]{{\ifcitation{\bibleftbracket#1\bibrightbracket}%
    {\bibleftparen#1\bibrightparen}}}
\renewcommand*{\bibopenparen}[1]{{\ifcitation{\bibleftbracket#1}{\bibleftparen#1}}}
\renewcommand*{\bibcloseparen}{{\ifcitation{\bibrightbracket}{\bibrightparen}}}
\appto\bibsetup{\raggedright}
\appto\bibfont{\LiningNumbers\small}

\addbibresource{Bibliography.bib}

